Osmotic forces modify lipid membrane fluctuations

In hydrodynamic descriptions of lipid bilayers, the membrane is often approximated as being impermeable to the surrounding, solute-containing fluid. However, biological and in vitro lipid membranes are influenced by their permeability and the resultant osmotic forces -- whose effects remain poorly understood. Here, we study the dynamics of a fluctuating, planar lipid membrane that is ideally selective: fluid can pass through it, while the electrically-neutral solutes cannot. We find that the canonical membrane relaxation mode, in which internal membrane forces are balanced by fluid drag, no longer exists over all wavenumbers. Rather, this mode only exists when it is slower than solute diffusion -- corresponding to a finite range of wavenumbers. The well-known equipartition result quantifying the size of membrane undulations due to thermal perturbations is consequently limited in its validity to the aforementioned range. Moreover, this range shrinks as the membrane surface tension is increased, and above a critical tension the membrane mode vanishes. Our findings are relevant when interpreting experimental measurements of membrane fluctuations, especially in vesicles at moderate to high tensions.

==> custom-commands.tex <==


% custom colors
\definecolor{myCyan}{rgb}{0.0, 0.47, 0.75}  \colorlet{myBlue}{blue!70!green}
\colorlet{myOrange}{red!60!yellow}          \colorlet{myRed}{orange!40!purple}
\colorlet{myGreen}{green!60!blue}           \colorlet{myPurple}{red!60!blue}
\colorlet{myDarkCyan}{myPurple!15!myCyan}

\definecolor{aOrange}{RGB}{191, 87, 0}


% reviewer edits
%\newcommand{\reva}[1]{\textcolor{myGreen}{#1}}
%\newcommand{\revb}[1]{\textcolor{magenta}{#1}}
%\newcommand{\both}[1]{\textcolor{myOrange}{#1}}			% add from both reviewers


% new square root definition
% from https://en.wikibooks.org/wiki/LaTeX/Mathematics#Roots
\def\sqrtl{\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
\setbox0=\hbox{$#1\sqrt{#2\,}$}\dimen0=\ht0
\advance\dimen0-0.15\ht0
\setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
{\box0\lower0.4pt\box2}}

% extend figure references
\newcommand{\figpart}[2]{\hyperref[#1]{\ref*{#1}(#2)}}


% total and partial derivatives
\newcommand{\dd}[2]{\dfrac{\md \mk {#1}}{\md \mk {#2}}}
\newcommand{\ddt}[2]{\dfrac{\md^2 \mk {#1}}{\md \mk {#2}^2}}
\newcommand{\pp}[2]{\dfrac{\partial \mk {#1}}{\partial \mk {#2}}}
\newcommand{\ppt}[2]{\dfrac{\partial^2 \mk {#1}}{\partial \mk {#2}^2}}
\newcommand{\ppth}[2]{\dfrac{\partial^3 \mk {#1}}{\partial \mk {#2}^3}}
\newcommand{\ppf}[2]{\dfrac{\partial^4 \mk {#1}}{\partial \mk {#2}^4}}


% operators
\newcommand{\bfrac}[2]{{^{#1} \! / \! _{#2}}} % in-text fractions
\newcommand{\bmcdot}{\bm{\cdot}}
\newcommand{\bmcolon}{\bm{:}}
\newcommand{\jj}[1]{\left\llbracket \mk #1 \mk \right\rrbracket} % jump quantity
\newcommand{\bmnabla}{\bm{\nabla}}
\newcommand{\bmnablaperp}{\bmnabla_{\!\! \perp}}
\newcommand{\bmnablapara}{\bmnabla_{\!\! \parallel}}
\newcommand{\pdp}{(\, \bmcdot \,)}


% bulk quantities
\newcommand{\cpm}{c^\pm}
\newcommand{\tilcp}{\tilc^{\, +}}
\newcommand{\tilcm}{\tilc^{\, -}}
\newcommand{\tilcpm}{\tilc^{\, \pm}}
\newcommand{\bmjpm}{\bmj^\pm}
\newcommand{\ppm}{p^\pm}
\newcommand{\tilpp}{\tilp^{\, +}}
\newcommand{\tilpm}{\tilp^{\, -}}
\newcommand{\tilppm}{\tilp^{\, \pm}}
\newcommand{\bmsigmap}{\bmsigma^+}
\newcommand{\bmsigmam}{\bmsigma^-}
\newcommand{\bmsigmapm}{\bmsigma^\pm}
\newcommand{\vpm}{v^\pm}
\newcommand{\vpmj}{\vpm_j}
\newcommand{\vpmk}{\vpm_k}
\newcommand{\bmvp}{\bmv^+}
\newcommand{\bmvm}{\bmv^-}
\newcommand{\bmvpm}{\bmv^\pm}
\newcommand{\tilvp}{\tilv^{\, +}}
\newcommand{\tilvm}{\tilv^{\, -}}
\newcommand{\tilvpm}{\tilv^{\, \pm}}
\newcommand{\tilvpmj}{\tilvpm_j}
\newcommand{\tilvpmk}{\tilvpm_k}
\newcommand{\tilvpmz}{\tilvpm_z}


% jump quantities
\newcommand{\jjc}{\jj{c}}
\newcommand{\jjp}{\jj{p}}


% material properties
\newcommand{\muf}{\mu^{}_{\mkern-1mu\text{f}}}
\newcommand{\nuf}{\nu^{}_{\mkern-1mu\text{f}}}
\newcommand{\nufsq}{\nu^{\, 2}_{\mkern-1mu\text{f}}}
\newcommand{\rhof}{\rho^{}_{\mkern-1mu\text{f}}}
\newcommand{\rhom}{\rho^{}_{\mkern-1mu\text{m}}}
\newcommand{\rhoeff}{\rho^{}_{\mkern-1mu\text{eff}}}
\newcommand{\lc}{\ell_{\text{c}}}


% frequencies
\newcommand{\omegaq}{\omega_{\bmq}}
\newcommand{\tilomegad}{\tilomega^{}_{\mkern-2mu\scriptscriptstyle D}}
\newcommand{\tilomegam}{\tilomega^{}_{\mkern-1mu\text{m}}}
\newcommand{\tilomegarho}{\tilomega^{}_{\mkern-2mu\rho}}
\newcommand{\omegaimp}{\omegaq^{\text{imp}}}
\newcommand{\omegam}{\omega^{}_{\mkern-1mu\text{m}}}
\newcommand{\omegamimp}{\omega^{\text{imp}}_{\mkern-1mu\text{m}}}
\newcommand{\omegarho}{\omega^{}_{\mkern-2mu\rho}}
\newcommand{\omegarhor}{\omega^{(\text{r})}_{\mkern-2mu\rho}}
\newcommand{\omegarhoimp}{\omega^{\text{imp}}_{\mkern-2mu\rho}}


% bifurcation parameters
\newcommand{\qz}{q_{0}}
\newcommand{\qzp}{\qz^+}
\newcommand{\qzm}{\qz^-}
\newcommand{\qzpm}{\qz^\pm}
\newcommand{\lambdacast}{\lambda_{\text{c}}^{\mkern-1mu\ast}}


% constant values at membrane surface
\newcommand{\barhq}{\bar{h}_{\bmq}}
\newcommand{\barc}{\bar{c}}
\newcommand{\barcp}{\barc^{\mk +}_{\bmq}}
\newcommand{\barcm}{\barc^{\mk -}_{\bmq}}
\newcommand{\barcpm}{\barc^{\mk \pm}_{\bmq}}
\newcommand{\barp}{\bar{p}}
\newcommand{\barpp}{\barp^{\mk +}_{\bmq}}
\newcommand{\barpm}{\barp^{\mk -}_{\bmq}}
\newcommand{\barppm}{\barp^{\mk \pm}_{\bmq}}
\newcommand{\barv}{\bar{v}}
\newcommand{\barvpa}{\barv^{\mk +}_{\alpha \mk \bmq}}
\newcommand{\barvma}{\barv^{\mk -}_{\alpha \mk \bmq}}
\newcommand{\barvpma}{\barv^{\mk \pm}_{\alpha \mk \bmq}}
\newcommand{\barvpz}{\barv^{\mk +}_{z \mk \bmq}}
\newcommand{\barvmz}{\barv^{\mk -}_{z \mk \bmq}}
\newcommand{\barvpmz}{\barv^{\mk \pm}_{z \mk \bmq}}


% normal mode quantities
\newcommand{\hatc}{\hat{c}}
\newcommand{\hatcp}{\hatc^{\mk +}_{\bmq}}
\newcommand{\hatcm}{\hatc^{\mk -}_{\bmq}}
\newcommand{\hatcpm}{\hatc^{\mk \pm}_{\bmq}}
\newcommand{\hath}{\hat{h}_{\bmq}}
\newcommand{\hathm}{\hath^{\text{m}}}
\newcommand{\hathrho}{\hath^\rho}
\newcommand{\hatl}{\hat{\lambda}_{\bmq}}
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatppm}{\hatp^{\mk \pm}_{\bmq}}
\newcommand{\hatu}{\hat{u}}
\newcommand{\hatum}{\hatu^{}_m}
\newcommand{\hatunm}{\hatu^{}_{-m}}
\newcommand{\hatumsq}{\lvert \hatu^{2}_m \rvert}
\newcommand{\hatv}{\hat{v}}
\newcommand{\hatva}{\hat{v}^{}_{\! \alpha \mk \bmq}}
\newcommand{\hatvx}{\hat{v}^{}_{\! x \mk \bmq}}
\newcommand{\hatvy}{\hat{v}^{}_{\! y \mk \bmq}}
\newcommand{\hatvpma}{\hat{v}^{\mk \pm}_{\! \alpha \mk \bmq}}
\newcommand{\hatvpmj}{\hat{v}^{\mk \pm}_{j \mk \bmq}}
\newcommand{\hatvpmz}{\hat{v}^{\mk \pm}_{z \mk \bmq}}


% hypothetical decomposition
\newcommand{\brc}{\breve{c}}
\newcommand{\chc}{\check{c}}


% wavenumbers
\newcommand{\barq}{\bar{q}}
\newcommand{\barbmq}{\bm{\barq}}
\newcommand{\qa}{q^{}_\alpha}
\newcommand{\qopt}{q^{}_{\text{opt}}} % optical wavenumber cutoff
\newcommand{\qx}{q^{}_x}
\newcommand{\qy}{q^{}_y}
\newcommand{\qxsq}{\qx{}^{\!\! 2}}
\newcommand{\lopt}{\ell_{\text{opt}}} % optical length cutoff


\newcommand{\kd}{k^{}_{\mkern-2mu\scriptscriptstyle D}}
\newcommand{\kdsq}{k^{\, 2}_{\mkern-2mu\scriptscriptstyle D}}
\newcommand{\knu}{k^{}_{\mkn \nu}}
\newcommand{\knusq}{k^{\, 2}_{\mkn \nu}}


% bending moduli
\newcommand{\kb}{k_{\text{b}}}
\newcommand{\kg}{k_{\text{g}}}


% experimental quantities
\newcommand{\asm}{a^{}_m}
\newcommand{\asmsq}{a^{\,\, 2}_m}
\newcommand{\bsm}{b^{}_m}
\newcommand{\bsmsq}{b^{\,\, 2}_m}
\newcommand{\csm}{c^{}_m}
\newcommand{\csmsq}{c^{\,\, 2}_m}
\newcommand{\mmax}{m^{}_{\text{max}}}
\newcommand{\rv}{r^{}_{\mkn\mkn \text{v}}}


% thermal energy
\newcommand{\kB}{k^{}_{\text{B}}}
\newcommand{\kBT}{\kB \vartheta}


% fluctuation spectra
\newcommand{\hqsq}{\langle \lvert \mk \tilhq \rvert^2 \rangle}
\newcommand{\hqsqequi}{\hqsq_{\text{equi}}}
\newcommand{\hqxsq}{\langle \lvert \mk \tilh_{\qx} \mkn \rvert^2 \rangle}
\newcommand{\hqxsqequi}{\hqxsq_{\text{equi}}}
\newcommand{\hqxsqexp}{\hqxsq_{\text{exp}}}

% thermal noise
\newcommand{\tilxiq}{\tilxi_{\bmq}}
\newcommand{\tilxiqp}{\tilxi_{\bm{q'}}}
\newcommand{\tilxiqr}{\tilxiq^{\mk(\text{r})}}
\newcommand{\tilxiqi}{\tilxiq^{\mk(\text{i})}}
\newcommand{\tilxiqpr}{\tilxiqp^{\mk(\text{r})}}
\newcommand{\tilxiqpi}{\tilxiqp^{\mk(\text{i})}}


% dimensionless numbers
\newcommand{\Pm}{\mcp} % permeability number
\newcommand{\Os}{\mcs} % osmotic number


% surface Laplacian
\newcommand{\Deltas}{\Delta_{\text{s}}}


% base state quantities
\newcommand{\cz}{c^{}_0}
\newcommand{\hz}{h^{}_0}
\newcommand{\hsz}{h^{}_\sz}
\newcommand{\lambdac}{\lambda^{}_{\text{c}}}
\newcommand{\lambdal}{\lambda^{}_{\ell}}
\newcommand{\lambdaz}{\lambda^{}_0}
\newcommand{\lambdasz}{\lambda^{}_\sz}
\newcommand{\pc}{p^{}_{\text{c}}}
\newcommand{\pz}{p^{}_0}
\newcommand{\sz}{{(0)}}


% text subscripts
\newcommand{\md}{\text{d}}
\newcommand{\smb}{{\text{b}}}
\newcommand{\smp}{{\text{p}}}


% tilde quantities
\newcommand{\tilc}{\tilde{c}}
\newcommand{\tileta}{\tilde{\eta}}
\newcommand{\tilf}{\tilde{f}}
\newcommand{\tilh}{\tilde{h}}
\newcommand{\tilhq}{\tilh_{\bmq}}
\newcommand{\tilj}{\tilde{j\mkern5mu}\mkern-5mu}
\newcommand{\till}{\tilde{\lambda}}
\newcommand{\tilomega}{\tilde{\omega}}
\newcommand{\tilp}{\tilde{p}}
\newcommand{\tilr}{\tilde{r}}
\newcommand{\tilsigma}{\tilde{\sigma}}
\newcommand{\tilv}{\tilde{v}}
\newcommand{\tilbmv}{\bm{\tilde{v}}}
\newcommand{\tilva}{\tilv^{}_\alpha}
\newcommand{\tilbmx}{\bm{\tilde{x}}}
\newcommand{\tilxi}{\tilde{\xi}}


% bold roman letters
\newcommand{\bma}{\bm{a}}
\newcommand{\bme}{\bm{e}}
\newcommand{\bmf}{\bm{f}}
\newcommand{\bmI}{\bm{I}}
\newcommand{\bmj}{\bm{j}}
\newcommand{\bmn}{\bm{n}}
\newcommand{\bmq}{\bm{q}}
\newcommand{\bmx}{\bm{x}}
\newcommand{\bmv}{\bm{v}}


% bold greek letters
\newcommand{\bmsigma}{\bm{\sigma}}


% math calligraphy
\newcommand{\mcp}{\mathcal{P}}
\newcommand{\mcs}{\mathcal{S}}
\newcommand{\scp}{\mathscr{P}}


% spacing
\newcommand{\mk}{\mkern1mu}
\newcommand{\mkn}{\mkern-1mu}
\newcommand{\qqquad}{\qquad\quad}
\newcommand{\qqandqq}{\qquad\text{and}\qquad}
\newcommand{\qqqandqqq}{\qqquad\text{and}\qqquad}
\newcommand{\qwhereq}{\quad\text{where}\quad}
\newcommand{\qqwhereqq}{\qquad\text{where}\qquad}
\newcommand{\qqqwhereqqq}{\qqquad\text{where}\qqquad}


% for edits
\newcommand{\as}[1]{\textcolor{red}{#1}}		% material to edit




